Modern Computer Arithmetic (version 0.5.1)

This is a draft of a book about algorithms for performing arithmetic, and their implementation on modern computers. We are concerned with software more than hardware - we do not cover computer architecture or the design of computer hardware. Instead we focus on algorithms for efficiently performing arithmetic operations such as addition, multiplication and division, and their connections to topics such as modular arithmetic, greatest common divisors, the Fast Fourier Transform (FFT), and the computation of elementary and special functions. The algorithms that we present are mainly intended for arbitrary-precision arithmetic. They are not limited by the computer word size, only by the memory and time available for the computation. We consider both integer and real (floating-point) computations. The book is divided into four main chapters, plus an appendix. Our aim is to present the latest developments in a concise manner. At the same time, we provide a self-contained introduction for the reader who is not an expert in the field, and exercises at the end of each chapter. Chapter titles are: 1, Integer Arithmetic; 2, Modular Arithmetic and the FFT; 3, Floating-Point Arithmetic; 4, Elementary and Special Function Evaluation; 5 (Appendix), Implementations and Pointers. The book also contains a bibliography of 236 entries, index, summary of notation, and summary of complexities.

==> acknowledge.tex <==
\chapter*{Acknowledgements} \label{acknowlegements}
\ifnotCUP{\addcontentsline{toc}{chapter}{Acknowledgements}}

We thank the French National Institute for Research in Computer Science and
Control (INRIA)\index{INRIA}, 
the Australian National University (ANU)\index{ANU}, 
and the Australian Research Council (ARC)\index{ARC}, 
for their support.  
The book could not have been written
without the contributions of many friends and colleagues, too numerous to
mention here, but acknowledged in the
text and in the \emph{Notes and References} sections at the end of each
chapter.
\thispagestyle{empty}

We also thank those who have sent us comments on and corrections to earlier
versions of this book:
J\"org Arndt\index{Arndt, J\"org}, %
Marco Bodrato\index{Bodrato, Marco}, %
Wolfgang Ehrhardt\index{Ehrhardt, Wolfgang} (with special thanks),
Steven Galbraith\index{Galbraith, Steven Douglas}, %
Torbj\"orn Granlund\index{Granlund, Torbj\"orn}, %
Guillaume Hanrot\index{Hanrot, Guillaume}, %
Marc Mezzarobba\index{Mezzarobba, Marc}, %
Jean-Michel Muller\index{Muller, Jean-Michel}, %
Denis Roegel\index{Roegel, Denis}, %
Wolfgang Schmid\index{Schmid, Wolfgang Alexander}, %
Arnold Sch\"on\-hage\index{Schonhage@{Sch\"onhage, Arnold}}, %
Sidi Mohamed Sedjelmaci\index{Sedjelmaci, Sidi Mohamed}, %
Emmanuel Thom\'e\index{Thome, Emmanuel@{Thom\'e, Emmanuel}}, %
and Mark Wezelenburg\index{Wezelenburg, Mark}. %
Two anonymous reviewers provided very helpful suggestions.

The \emph{Mathematics Genealogy Project}\index{Mathematics Genealogy
Project} (\url{http://www.genealogy.ams.org/}) 
and Don Knuth's\index{Knuth, Donald Ervin}
\emph{The Art of Computer Programming}~\cite{Knuth98}
were useful resources for details of entries in the index.

We also thank the authors of the \LaTeX\ program, which allowed us to produce
this book, the authors of the \texttt{gnuplot}\index{gnuplot} program, 
and the authors of the GNU MP library,\index{GMP} which
helped us to illustrate several algorithms with concrete figures.

Finally, we acknowledge the contribution of 
Erin Brent,\index{Brent, Erin Margaret} 
who first suggested writing the book;
and thank our wives, Judy-anne\index{Osborn, Judy-anne Heather} 
and Marie,\index{Zimmermann, Marie}
for their patience and encouragement.


==> preface.tex <==
\chapter*{Preface} \label{preface}
\ifnotCUP{\addcontentsline{toc}{chapter}{Preface}\vspace*{-10pt}}

This is a book about algorithms for performing arithmetic, and their
implementation on modern computers.  We are concerned with software more
than hardware --- we do not cover computer architecture or the design of
computer hardware since good books are already available on these topics.
Instead we focus on algorithms for efficiently performing arithmetic
operations such as addition, multiplication and division, and their
connections to topics such as modular arithmetic, greatest common divisors,
the Fast Fourier Transform (FFT), and the computation of special functions.
\thispagestyle{empty}	%

The algorithms that we present are mainly intended for arbitrary-precision
arithmetic. That is, they are not limited by the computer wordsize of $32$
or $64$ bits, only by the memory and time available for the computation.
We consider both integer and real (floating-point) computations.

The book is divided into four main chapters, plus one short
chapter (essentially an appendix). 
Chapter \ref{integer}
covers integer arithmetic. This has, of course, been considered in
many other books and papers.
However, there has been much
recent progress, inspired in part by the application to public key
cryptography, so most of the published books are now partly out of date or
incomplete. Our aim is to present the latest developments in a concise
manner. At the same time, we provide a self-contained introduction for the
reader who is not an expert in the field.

Chapter \ref{modular} is concerned with modular arithmetic and the FFT, 
and their applications to computer arithmetic. We consider different number
representations, fast algorithms for multiplication, division and 
exponentiation, and the use of the Chinese Remainder Theorem (CRT).

\ifnotCUP{\begin{samepage}}
Chapter \ref{float} covers floating-point arithmetic. Our concern is with
high-{\lbrkc}precision 
floating-point arithmetic, implemented in software if the
precision provided by the hardware (typically IEEE standard $53$-bit
significand) is{\lbrkc} inadequate. 
The algorithms described in this chapter focus on
\emph{correct rounding}, extending the IEEE standard to arbitrary precision.
\ifnotCUP{\end{samepage}\pagebreak[3]}

Chapter \ref{special} deals with the computation, to arbitrary precision, of
functions such as sqrt, exp, ln, sin, cos, and more generally
functions defined by power series or continued fractions. 
Of course, the computation of special functions
is a huge topic so we have had to be selective. In particular, we have
concentrated on methods that are efficient and suitable for
arbitrary-precision computations. 

The last chapter contains pointers to
implementations, useful web sites, mailing lists, and so on.
Finally, at the end there is a one-page \emph{Summary of Complexities}
which should be a useful \emph{aide-m\'emoire}.

The chapters are fairly self-contained, so it is possible to read them out of
order.  For example, Chapter 4 could be read before Chapters 1--3, and 
Chapter 5 can be consulted at any time. Some
topics, such as Newton's method, appear in different guises in several
chapters. Cross-references are given where appropriate.

For details that are omitted we give pointers in the \emph{Notes and
References} sections of each chapter, as well as in the bibliography.
We have tried, as far as possible, to keep the main text uncluttered by 
footnotes and references, so most references are given in the
\emph{Notes and References} sections.

The book is intended for anyone interested in the design and implementation
of efficient algorithms for computer arithmetic, and more generally
efficient numerical algorithms. We did our best to present
algorithms that are ready to implement in your favorite
language, while keeping a high-level description and not getting
too involved in low-level or machine-dependent details.
An alphabetical list of algorithms can be found in the index.

Although the book is not specifically intended
as a textbook, it could be used in a graduate course in mathematics or
computer science, and for this reason, as well as to cover topics that could
not be discussed at length in the text, we have included exercises at the
end of each chapter. The exercises vary considerably in difficulty, from 
easy to small research projects, but we have not attempted to assign them
a numerical rating. For solutions to the exercises, please contact the authors.


\medskip
\emph{We welcome comments and corrections. 
Please send them to either of the authors.}
\bigskip

\rightline{Richard Brent and Paul Zimmermann}
\rightline{\texttt{MCA@rpbrent.com}}\index{email addresses}
\rightline{\texttt{Paul.Zimmermann@inria.fr}}
\rightline{Canberra and Nancy, February 2010}

